Characterizing Input Methods for Human-to-robot Demonstrations

Human demonstrations are important in a range of robotics applications, and are created with a variety of input methods. However, the design space for these input methods has not been extensively studied. In this paper, focusing on demonstrations of hand-scale object manipulation tasks to robot arms with two-finger grippers, we identify distinct usage paradigms in robotics that utilize human-to-robot demonstrations, extract abstract features that form a design space for input methods, and characterize existing input methods as well as a novel input method that we introduce, the instrumented tongs. We detail the design specifications for our method and present a user study that compares it against three common input methods: free-hand manipulation, kinesthetic guidance, and teleoperation. Study results show that instrumented tongs provide high quality demonstrations and a positive experience for the demonstrator while offering good correspondence to the target robot.

==> 7_conclusion.tex <==
\section{CONCLUSION}

In this paper, we have presented a design study of input devices for obtaining human demonstrations for robotics applications. We examined a range of use cases to derive a set of features that serve as a design space to place designs. We examined the main existing input methods to understand their benefits and drawbacks. We introduced a design for a new input device, \emph{instrumented tongs,} motivated by the needs of use cases involving obtaining data from inexperienced users performing object manipulation tasks. 

We performed an evaluation of the tongs that show they provide quality movements in demonstrations, a desirable user experience for the demonstrator, acceptable mapping to the target robot, and are practical to instrument. A human subjects study suggests that the tongs are competitive with the best existing devices for each of these attributes, but uniquely provide good performance on all. Ultimately, our best evidence for the efficacy of the tongs will be their success in real use cases. 
Already, we have seen new techniques 
(citations redacted to maintain anonymity)
%(e.g., \cite{guru-IROS2017, guruICRA2018, guruCORL2018, guruICRA2019}) 
enabled by the tongs' combination of practicality, instrumentability, usability, and demonstration quality.


